OOD-DiskANN: Efficient and Scalable Graph ANNS for Out-of-Distribution Queries

State-of-the-art algorithms for Approximate Nearest Neighbor Search (ANNS) such as DiskANN, FAISS-IVF, and HNSW build data dependent indices that offer substantially better accuracy and search efficiency over data-agnostic indices by overfitting to the index data distribution. When the query data is drawn from a different distribution - e.g., when index represents image embeddings and query represents textual embeddings - such algorithms lose much of this performance advantage. On a variety of datasets, for a fixed recall target, latency is worse by an order of magnitude or more for Out-Of-Distribution (OOD) queries as compared to In-Distribution (ID) queries. The question we address in this work is whether ANNS algorithms can be made efficient for OOD queries if the index construction is given access to a small sample set of these queries. We answer positively by presenting OOD-DiskANN, which uses a sparing sample (1% of index set size) of OOD queries, and provides up to 40% improvement in mean query latency over SoTA algorithms of a similar memory footprint. OOD-DiskANN is scalable and has the efficiency of graph-based ANNS indices. Some of our contributions can improve query efficiency for ID queries as well.

==> algorithms/5-increment-key.tex <==
\begin{algorithm}
\caption{\incrementkey($v$)}
\label{alg:increment-key}
\DontPrintSemicolon
\small
\SetKwFunction{FKeys}{keys}
\SetKwFunction{FGet}{get\_count}
\SetKwFunction{FInsert}{insert}
\SetKwFunction{FDelete}{delete}
\KwData{Max heap $\mathcal{H}$ and graph node $v$.}
\KwResult{Updated max heap.}
\Begin{
    \eIf{$v \in \mathcal{H}$.\FKeys{}}{
        \nonl $v_{\text{count}} \leftarrow \mathcal{H}.$\FGet{$v$}\;
        \nonl $\mathcal{H}.$\FDelete{$v$} $; \mathcal{H}.$\FInsert{$v, v_{\text{count}} + 1$}\;
    }{
        \nonl $\mathcal{H}.$\FInsert{$v, 1$}\;
    }
}
\end{algorithm}

==> algorithms/6-random-seed.tex <==
\begin{algorithm}
\caption{\randomseed($\mathcal{D}$)}
\label{alg:random-seed}
\DontPrintSemicolon
\small
\SetKwFunction{FKeys}{keys}
\KwData{Bitmap $\mathcal{D}$ of already packed nodes.}
\KwResult{A random unpacked seed node $s$.}
\Begin{
    \For{$s \in \mathcal{D}$.\FKeys{}}{
        \If{{\normalfont not} $ \mathcal{D}[s]$}{
            \nonl $\mathcal{D}[s] \leftarrow \text{true}$\;
            \KwRet $s$\;
        }
    }
    
}
\end{algorithm}

==> algorithms/9-query-select.tex <==
\begin{algorithm}[t]
\caption{Query Set Selection Algorithm}
\label{alg:query-set-select}
\DontPrintSemicolon
\small
\KwData{Number of closest base points to retrieve per query $T$, max number of queries per base point $Q_{\text{max}}$,
distance metric}
\KwResult{Sample query sets $\mathcal{Q}_{x_{i}}$ pertaining to each base point $x_{i}$.}
\Begin{
    \For{$q_{i} \in \mathcal{Q}$}{
        \nonl Let $\mathcal{T}$ be the $T$ closest points in index to $q_{i}$\;
        \For{$x_{i} \in \mathcal{T}$}{
            \If{$|\mathcal{Q}_{x_{i}}| < Q_{\text{max}}$}{
                \nonl $\text{Update } \mathcal{Q}_{x_{i}} \leftarrow \mathcal{Q}_{x_{i}} \cup q_{i}$\;
            }
        }
    }
}
\end{algorithm}

==> sections/accurate-product-quantization.tex <==
% \section{Compression with Accurate Product Quantization}
% \label{sec:accurate-product-quantization}

% % Give high level problem overview.
% Graph ANNS is completely guided by the distance estimates between the query and the base dataset nodes encountered along the graph traversal. Highly accurate estimates allow the search algorithm to discern the near neighbors and correctly rank their closeness to a query, leading to higher recall.

% Base dataset vectors need to be RAM-resident for quickly computing the distances. Loading the original vectors, which provide the most accurate estimates, becomes unviable for high-dimensional large-scale datasets because of RAM constraints. As such, existing systems make use of a two-stage shortlisting and re-ranking approach for their search. In particular, \previoustool makes use of Product Quantization (PQ) to compress the base dataset vectors to a suitable size, loads them into the RAM, and makes use of these compressed vectors to obtain approximate distance estimates during graph traversal. Based on these estimates, it shortlists a candidate set of nearest neighbors. Since the number of shortlisted candidates is much smaller than the total number of candidates explored in this process, only a small number of original vectors need to be loaded into memory for more accurate distance estimation and re-ranking. This is achieved by storing the original vectors on the disk, and paging them into RAM through I/O requests, after shortlisting. The final re-ranked set is returned as the result of the query search.

% For any variant of PQ, the accuracy of distance estimates is primarily determined by two factors, namely the compression ratio and the quality of compression. The former refers to the ratio of the byte-size of the original vector to the byte-size of the PQ bit-codes for that vector. Since PQ is a lossy scheme, a higher compression ratio leads to a lower RAM footprint, but incurs heavier distortions in its distance estimates. Quality of compression refers to the ability of the PQ-generated pivots to accurately represent the data being compressed, which is the core area of improvement in our work.

% Once the RAM-resident vectors are compressed using PQ pivots, we typically have two choices for approximating the distance between the query and the base points:

% \textbf{Symmetric Distance Computation (SDC):} Both the base and the query vectors ($x_{i}$ and $q$ respectively) are represented by their most suitable pivots ($\mu_{x_{i}}$ and $\mu_{q}$ respectively), and the distance between these pivots is approximated to be the distance between $x_{i}$ and $q$.

% \textbf{Asymmetric Distance Computation (ADC):} Only the base vector ($x_{i}$) is represented by its most suitable pivot ($\mu_{x_{i}}$), and the distance between $x_{i}$ and $q$ is approximated to be the distance between $\mu_{x_{i}}$ and $q$.

% ANNS algorithms utilizing any flavor of PQ compression unequivocally compute ADC because of the lower distance distortion incurred, compared to SDC. As such, during the shortlisting stage, we compute the ADC estimate by summing up the chunk-wise distances between the query vector chunk $q_{j[:]}$ and pivot $\mu_{x_{i, j[:]}}$ assigned to base sub-vector $x_{i, j[:]}$ for a given chunk index $j$.

% \subsection{ADC Analysis for Euclidean Metric}
% For the euclidean metric, given vectors $q, x_{i} \in \mathbb{R}^{D}$ with $x_{i}$ chunked into $M$ sub-vectors, we have:
% \begin{flalign} \label{eq:1}
%     \underbrace{\|q - x_{i}\|^{2}_{2}}_{\text{True Distance}} & = \sum_{j=1}^{M}\underbrace{\|q_{j[:]} - x_{i, j[:]}\|^{2}_{2}}_{\text{Chunk True Distance}} \nonumber \\ & = \sum_{j=1}^{M}\|q_{j[:]} - \mu_{x_{i, j[:]}} + \mu_{x_{i, j[:]}} - x_{i, j[:]}\|^{2}_{2} &&
% \end{flalign}
% \begin{flalign} \label{eq:2}
%     \underbrace{\|q - x_{i}\|^{2}_{2}}_{\text{True Distance}} = & \sum_{j=1}^{M}[\underbrace{\|q_{j[:]} - \mu_{x_{i, j[:]}}\|^{2}_{2}}_{\text{Chunk ADC Estimate}} + \text{ }\|x_{i, j[:]} - \mu_{x_{i, j[:]}}\|^{2}_{2} \nonumber \\ & - 2 \langle q_{j[:]} - \mu_{x_{i, j[:]}}, x_{i, j[:]} - \mu_{x_{i, j[:]}} \rangle] &&
% \end{flalign}
% Using equation (\ref{eq:1}) and (\ref{eq:2}), we calculate the distortion between the true distance and the ADC estimate as:
% \begin{flalign} \label{eq:3}
%     & \sum_{j=1}^{M}[\underbrace{\|q_{j[:]} - x_{i, j[:]}\|^{2}_{2}}_{\text{Chunk True Distance}} - \underbrace{\|q_{j[:]} - \mu_{x_{i, j[:]}}\|^{2}_{2}}_{\text{Chunk ADC Estimate}}] \nonumber \\
%     % & = \sum_{j=1}^{M}[\|x_{i, j[:]} - \mu_{x_{i, j[:]}}\|^{2}_{2} \\ & \quad \quad \quad- 2 \langle q_{j[:]} - \mu_{x_{i, j[:]}}, x_{i, j[:]} - \mu_{x_{i, j[:]}} \rangle] \\ 
%     & = \sum_{j=1}^{M}[\langle x_{i, j[:]} - \mu_{x_{i, j[:]}}, x_{i, j[:]} - \mu_{x_{i, j[:]}} \rangle \nonumber \\ & \quad \quad \quad \quad - 2 \langle q_{j[:]} - \mu_{x_{i, j[:]}}, x_{i, j[:]} - \mu_{x_{i, j[:]}} \rangle] &&
% \end{flalign}
% Continuing on equation (\ref{eq:3}), and taking the ($x_{i, j[:]} - \mu_{x_{i, j[:]}}$) vector common across inner products:
% \begin{flalign} \label{eq:4}
%     & \sum_{j=1}^{M}[\underbrace{\|q_{j[:]} - x_{i, j[:]}\|^{2}_{2}}_{\text{Chunk True Distance}} - \underbrace{\|q_{j[:]} - \mu_{x_{i, j[:]}}\|^{2}_{2}}_{\text{Chunk ADC Estimate}}] \nonumber \\ & = \sum_{j=1}^{M}\langle x_{i, j[:]} + \mu_{x_{i, j[:]}} - 2q_{j[:]},  x_{i, j[:]} - \mu_{x_{i, j[:]}} \rangle &&
% \end{flalign}
% Hence equation (\ref{eq:4}) depicts the total distortion between the true distance and the ADC estimate values for a given query and base vector pair, as a sum of chunk-wise inner products. A positive value of the distortion term signifies that the base point appears closer to the query than it actually is, and likewise, a negative value of distortion term signifies that the base point appears further away.

% Looking at the distortion term for the $j$-th chunk, we can simplify the above as:
% \begin{flalign} \label{eq:5}
%     & \langle x_{i, j[:]} + \mu_{x_{i, j[:]}} - 2q_{j[:]},  x_{i, j[:]} - \mu_{x_{i, j[:]}} \rangle \nonumber \\ & = \frac{1}{2}\|\frac{x_{i, j[:]} + \mu_{x_{i, j[:]}}}{2} - q_{j[:]}\|_{2} \|x_{i, j[:]} - \mu_{x_{i, j[:]}}\|_{2}\cos{\theta} &&
% \end{flalign}
% where, $\theta$ is the angle between the above two inner product vectors.

% % Explain what existing solutions do.
% Here, the first multiplicative term is equal to the euclidean distance between a given query sub-vector and the mid-point between a base sub-vector and the pivot assigned to it. Existing PQ schemes only aim to minimize the squared euclidean norm of the second multiplicative term as an upper-bound of the overall distortion.

% In order to remedy this issue, we propose Accurate Product Quantization (APQ), where we directly minimize the distortion between the true distance and the ADC estimate, by considering it as a loss objective for generating our PQ pivots. As this objective is dependent upon a given query and base vector pair, we again make the relaxing assumption that a small set of independently sampled queries is available to us. PQ-based methods are extremely tolerant to sub-sampling, and as such we don't require a sample set of more than $100$K queries and $100$K base points, both randomly sampled without replacement.

% Not all query-base pairs are equally important, since very few base points are commonly visited across different query search paths. For each sample query, one needs to only focus on the set of base points which are in close proximity to it, and vice versa. Hence, for each base point $x_{i}$, we define a set of relevant sample queries $\mathcal{Q}_{x_{i}}$ as described in \textbf{\autoref{alg:query-set-select}}.

% \input{algorithms/9-query-select}

% We then define our loss function for euclidean metric $\mathcal{L}_{\text{APQ-L$2$}}$:

% \begin{flalign}\label{eq:8}
%     & \mathcal{L}_{\text{APQ-L$2$}}(x_{i, j[:]}, \mu, \mathcal{Q}_{x_{i}}) \nonumber \\ & = \frac{1}{|\mathcal{Q}_{x_{i}}|} \sum_{q \in \mathcal{Q}_{x_{i}}}
%         \begin{cases}
%             -\langle x_{i, j[:]} + \mu - 2q_{j[:]},  x_{i, j[:]} - \mu \rangle, & \text{if}\ x_{i} \in \text{H}(q) \\
%             |\langle x_{i, j[:]} + \mu - 2q_{j[:]},  x_{i, j[:]} - \mu \rangle|, & \text{otherwise}
%         \end{cases} &&
% \end{flalign}
% where, $\mu \in \mathbb{R}^{\frac{D}{M}}$ is a pivot and $\text{H}(q)$ is the set of $k$ closest base points to $q$. This way of formulating the loss objective is inspired from previous works employing contrastive loss. In the first case, we force the optimizer to minimize the negative distortions, and amplify the positive distortions, for a select subset of relevant queries which are known to be really close. In the second case, we force the optimizer to minimize the magnitude of the distortions themselves for the rest.

% % Explain the solution.
% We optimize this loss objective (\ref{eq:8}) and (\ref{eq:13}) through an alternating minimization approach. \textbf{\autoref{alg:chunk-wise-accurate-pq}} and \textbf{\autoref{alg:accurate-pq-codebook-learning}} summarise our approach where we partition our base dataset into $M$ chunks, and learn a set of $k$ independent pivots for each chunk. We initiate the learning process for a chunk by choosing a random set of $k$ pivot points, and follow up with membership assignment and pivot update steps in an alternating fashion. The learnt set of pivots pertaining to the $j$-th chunk form a dictionary $C_{j}$, and the final set of $M$ dictionaries form our learnt codebook $\mathcal{C}$. This codebook is then used to encode the original base dataset vectors.

% \input{algorithms/10-accurate-pq}

% \input{algorithms/11-codebook-learning}

% \begin{figure*}
% \flushleft
% \begin{minipage}{\columnwidth}
%     \input{figures/combined-apq}
% \end{minipage}
% \caption{(Left to right) Latency vs.\ Recall for Web Ads, Yandex T2I and Turing T2I (10M scale).}
% \label{fig:combined-apq}
% \end{figure*}

% As evident from \textbf{\autoref{fig:combined-apq}}, we observe a $3-4\%$ improvement in recall, for the same latency target, in the case of OOD datasets. We also observe a negligible change in performance for the ID Web Ads dataset. Since we need to construct query sets for each base point, we have a disk space overhead of roughly 400 bytes per base point (for storing roughly 100 query ids). Additionally, we train Accurate PQ through gradient descent, which takes roughly $1$ minute per chunk using Tensorflow on CPU.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. Please read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/graph-reordering.tex <==
% \section{\parallelgorder Graph Reordering}
% \label{sec:graph-reordering}
% % Give high level problem overview.
% Graph-based ANNS algorithms, at their core, traverse nodes in the graph in a locally-greedy manner -- walking over to the node closest to query in the adjacency list of the current node -- during search. At every node, accessing the adjacency is a random access that is likely to be a cache miss given that the graph traversal happens in a high dimensional space with no linear projection onto a one-dimensional virtual address space. Further, a node once referenced is never referenced again for that query. This means that greedy graph traversal have poor inherent locality.

% % Give more details.
% % Explain what existing solutions do.
% However, there is some work on graph reordering methods  to improve search latency to a limited extent by placing information regarding nodes likely to be referenced together while serving  on the same or adjacent  cache lines (which can be prefetched efficiently by the CPU instruction pipeline).  This has the effect of reducing the number of cache misses incurred during graph traversal, as one needs fewer cache line transfers to page in the same set of referenced nodes. \citet{coleman-survey} have surveyed several reordering techniques applied to the \hnsw algorithm, and consistently observed the best speedups with \gorder algorithm for in-memory graph ANNS.

% % Explain what Gorder is.
% \gorder proposes that nodes ``local'' to each other  should be placed next to one another in the storage layout. The locality of a pair of nodes is estimated by counting the number of common in-neighbors and  directed edges between the nodes. \gorder algorithm aims to find a graph ordering that maximizes the sum of locality scores over a fixed-size rolling window, that corresponds to a hardware unit of access (e.g. cache line). \gorder works well in the case of ANNS because, more often than not, a node being referenced during search is either a neighbor or a sibling of a recently referenced node.

% \input{figures/ordering_example}

% % Show how it's applicable to our use case.
% \textbf{Locality for External Memory:} Indexing large datasets requires indices that need to be stored on Solid State Drives (SSD). Search performance for such disk-based indices search is bottlenecked by maximum number of random IOs per second supported by the SSD. Waiting on such IO  typically accounts for more than $50\%$ of the overall latency for \previoustool even when used with a newer NVMe (Non-Volatile Memory Express) SSDs. Quite naturally, it can benefit significantly from reduced I/O requests through disk layout reordering.

% We make the observation that these indices typically store graph nodes in fixed-size (usually $4$KBs) disk sectors. For \previoustool, each sector contains as many nodes as can be placed completely within it. Hence, an I/O  typically fetches more than one node from the disk for no extra overhead. Through reordering, we wish to exploit this property. 
% %Fetching a node from disk requires one to identify the disk sector containing the node, and issue an I/O request for that sector.

% % Show why one needs to adapt the existing solutions.
% However, vanilla \gorder is ill-suited for this task, since it has a high cost ($\mathcal{O}(NR^{2})$ where $N$ denotes the number of graph nodes, and $R$ denotes the maximum out-degree) and the sliding window-based computation of \gorder (called {\em GO-PQ}) is non-parallelizable.  The total build-time cost which is empirically $1.5\text{ - }2\times$ higher the index construction, and cannot be parallelized, is not practical. %, since graph-based methods have a rough build-time cost of $\mathcal{O}(NRD)$, where $D$ denotes the dimensionality of the dataset vectors. 

% % Additionally, unlike the in-memory scenario where all the CPU search threads access a single unified L3 cache, I/O search threads make use of individual, non-cached I/O buffers while paging in sectors from the disk, to prevent concurrency issues from arising.

% % \input{algorithms/5-increment-key}
% % \input{algorithms/6-random-seed}
% \input{algorithms/7-parallel-gorder}
% \input{algorithms/8-sector-pack}

% % Explain the solution.
% Since SSD read latencies are impartial to random vs.\ sequential sector fetches, one only needs to maximise the locality between all the graph nodes stored in a particular disk sector, without worrying about the locality of nodes spread across two different sectors. This opens up the possibility to ``pack'' each sector with nodes individually, making the entire process parallelizable. In case of a race condition, where a node has multiple different sectors where it can be packed into, we simply choose a sector at random for the node to stored into, and re-initiate the packing process on the rest.

% \textbf{\autoref{alg:parallel-gorder}} and \textbf{\autoref{alg:sector-pack}}  describe our approach, where we make use of a standard max heap for tracking the most suitable node to add to a partially-packed sector, starting with a randomly-chosen seed node. Note that using a max heap pushes the runtime of our algorithm to $\mathcal{O}(NR^{2}\log{R})$, which is only slightly worse than the original, non-parallel algorithm since $R$ is typically $< 150$.

% \begin{figure*}
% % \flushleft
% % \begin{minipage}{\columnwidth}
% %     \input{figures/combined-reorder-io}
% % \end{minipage}
% % \vfill
% \flushleft
% \begin{minipage}{\columnwidth}
%     \input{figures/combined-reorder-latency}
% \end{minipage}
% \caption{(Left to right) Latency vs.\ Recall for Web Ads, Yandex T2I and Turing T2I (10M scale).}
% \label{fig:combined-reorder-io-latency}
% \end{figure*}

% % We implement per-thread I/O caches in RAM, which store the sectors paged in from the disk by the associated search thread, and remove the existing non-cached I/O buffers. This leads to zero change in RAM footprint during search time, while ensuring efficient I/O re-use. 

% For floating-point datasets, we also quantize the original, single-precision ($32$-bit) dataset vectors into unsigned ($8$-bit) integer vectors of the same dimensionality, using the vanilla PQ algorithm. These $4\times$ compressed vectors are stored in place of the original float vectors on the disk. This integer quantization leads to minimal recall loss during final re-ranking of candidate nearest neighbors, while allowing us to pack a higher number of nodes in a single disk sector, as the node now occupies fewer bytes of space.

% % Explain the net result, and show why it's unique.
% We observe anywhere from $15\text{ - }40\%$ reduction in I/O requests. As evident from \textbf{\autoref{fig:combined-reorder-io-latency}}, this leads to $10\text{ - }25\%$ improvement in mean latency, in the high recall regime. These gains are obtained with roughly a $7\text{ - }12\%$ increase in build-time, keeping the peak RAM and disk usage unchanged during both the build and search.

% % We consciously avoid implementing a thread-safe unified I/O cache because we observed poor empirical performance. This was due to high lock contention arising from concurrency checks needed to prevent race conditions during search. First In First Out (FIFO) eviction strategy was used, in place of a more popular Least Recently Used (LRU) strategy, because the former offers a lower compute overhead, with negligible impact on cache hits in our experiments.
